Equivalence Checking and Simulation By Computing Range Reduction

We introduce new methods of equivalence checking and simulation based on Computing Range Reduction (CRR). Given a combinational circuit $N$, the CRR problem is to compute the set of outputs that disappear from the range of $N$ if a set of inputs of $N$ is excluded from consideration. Importantly, in many cases, range reduction can be efficiently found even if computing the entire range of $N$ is infeasible. Solving equivalence checking by CRR facilitates generation of proofs of equivalence that mimic a "cut propagation" approach. A limited version of such an approach has been successfully used by commercial tools. Functional verification of a circuit $N$ by simulation can be viewed as a way to reduce the complexity of computing the range of $N$. Instead of finding the entire range of $N$ and checking if it contains a bad output, such a range is computed only for one input. Simulation by CRR offers an alternative way of coping with the complexity of range computation. The idea is to exclude a subset of inputs of $N$ and compute the range reduction caused by such an exclusion. If the set of disappeared outputs contains a bad one, then $N$ is buggy.

==> e3c_cut1.fig.tex <==
\setlength{\intextsep}{4pt}
\begin{wrapfigure}{l}{1.7in}
%\begin{figure} 
 \begin{center}
    \includegraphics[width=1.7in]{ee3c_cut1.jpg}
  \end{center}
\caption{A cut formed by equivalent internal points of $N'$ and $N''$}
\label{fig:ec_cut1}
%\end{figure}
\end{wrapfigure}


==> junk.tex <==
\vspace{50pt}
dfdfdfdf
\clearpage
dffdfdfd
\clearpage


==> more_detail.tex <==
\section{High-level description of equivalence checking and simulation by CRR}
\subsection{Equivalence checking and CRR}
Let $N'(X',Y',z')$ and $N''(X'',Y'',z'')$ be two single-output
combinational circuits whose equivalence one needs to establish.
(Here we slightly abuse terminology by using term ``output'' to denote
an output variable of $N$.  So the term ``single-output circuit''
implies that this circuit has only one output variable. Whether we
mean an ``output variable'' or an ``output assignment'' should be
clear from the context.) The best commercial tools are very effective
in reducing the complexity of Equivalence Checking (EC) when circuits
$N'$ are $N''$ are structurally similar i.e.  have many functionally
equivalent subcircuits.  In this case, equivalence of $N'$ and $N''$
is performed in terms of cut variables rather than input variables
$X$.


Figure~\ref{fig:ec_cut1} gives circuits $N'$ and $N''$ and a cut shown
in the dotted line. This cut consists of points of $N'$ and $N''$ that
are functionally equivalent. For example, variables $y'$ and $y''$
specify outputs of subcircuits of $N'$ and $N''$ proved equivalent.  So
the proof of equivalence of $N'$ and $N''$ looks like advancing cuts
from inputs $X$ to outputs $z'$ and $z''$ (see
Figure~\ref{fig:ec_cut2}).  First, internal variables of $N'$ and
$N''$ are proved equivalent in terms of cut $\mi{Cut}_1$. Then
internal variables of cut $\mi{Cut}_2$ are proved equivalent in terms
of cut $\mi{Cut}_1$ and so on.

\input{e3c_cut1.fig} 

Unfortunately, the requirement for $N'$,$N''$ to have many
functionally equivalent internal points is very restrictive.  One can
give examples of circuits that do not have functionally equivalent
internal points being very structurally similar~\cite{int_ext}.
Intuitively, such circuits can be checked for equivalence by a
generalized version of the cut advancement method. In this version,
structurally similar internal points of $N'$ and $N''$ are related by
short clauses (but these clauses do not have to specify equivalence of
internal points). These ``relation clauses'' are computed in
topological order from inputs to outputs.

Instead of using dedicated EC algorithms, one can reduce equivalence
checking to SAT and apply a SAT-solver based on Conflict Driven Clause
Learning (CDCL)~\cite{grasp,chaff}.  The problem however is that
CDCL solvers generate ``unstructured'' proofs and hence can be very
inefficient in comparison to methods employing a cut advancement
strategy. To follow such a strategy, a CDCL solver needs to derive
meaningful conflict clauses relating structurally close points of $N'$
and $N''$. However, it is not clear how one can make a CDCL
solver do that.


We argue that EC by CRR can address the problem above. In particular,
EC by CRR facilitates generation of clauses that relate variables of
$N'$ and $N''$. Moreover, an equivalence checker performing CRR can
potentially mimic the cut advancement strategy even when circuits $N'$
and $N''$ do not have any functionally equivalent internal points.

Application of CRR to EC is based on the following observation. Let
$N'$ and $N''$ be single-output combinational circuits to be checked
for equivalence. Let $M$ be a two-output circuit composed of $N'$ and
$N''$ as shown in Figure~\ref{fig:two_indep}.  Note that the sets $X'$
and $X''$ of input variables of $N'$ and $N''$ are independent of each
other.  Then, if $N'$ and $N''$ are not constants, the range of
circuit $M$ consists of all four assignments to variables $z'$,$z''$
specifying the outputs of $N'$ and $N''$. Let (\pnt{x'},\pnt{x''})
denote an assignment to variables $X' \cup X''$. Suppose that one
excludes from consideration all assignments (\pnt{x'},\pnt{x''}) where
$\pnt{x'} \neq \pnt{x''}$. Then if $N'$ and $N''$ are functionally
equivalent, such constraint on inputs of $M$ should lead to
disappearing assignments $(z'=0,z''=1)$ and $(z'=1,z''=0)$ from the
range of $M$. If this is not the case, then there is an input
(\pnt{x'},\pnt{x''}) of $M$ where \pnt{x'}=\pnt{x''} for which $N'$
and $N''$ evaluate to different values i.e.  $N'$ and $N''$ are not
functionally equivalent.

The claim that EC by CRR facilitates a cut propagation strategy is
based on the following intuition. In~\cite{tech_rep_crr} we showed
that CRR comes down to Partial Quantifier Elimination (PQE). Denote by
$G(X',X'')$ a set of clauses that excludes the inputs of $M$ for which
$\pnt{x'} \neq \pnt{x''}$. In terms of PQE, the EC problem is to
derive clauses containing variables $z',z''$ that make the clauses of
$G$ redundant. The problem of making clauses of $G$ redundant can be
partitioned into subproblems.  First, clauses $G_1$ relating points of
some cut $\mi{Cut}_1$ of $N'$ and $N''$ are derived that make the
clauses of $G$ redundant. Then clauses $G_2$ relating points of cut
$\mi{Cut}_2$ are generated that make the clauses of $G_1$ redundant
and so on until the cut consisting of variables $z',z''$ is reached.


\subsection{Application of CRR to simulation-by-exclusion}
\label{subsec:intr_sim_by_excl}
Computing the range of a combinational circuit $N(X,Y,Z)$ is an
important verification problem. For instance, Circuit-SAT can be
viewed as computing the range of $N$ when $|Z|=1$. In general,
computing the range of $N$ is a hard problem.  Simulation can be viewed
as a way to simplify it by computing the range of $N$ only
for one input (regular simulation) or for a subset of inputs (symbolic
simulation~\cite{SymbolSim}).

In this paper, we consider a different way to cope with complexity of
range computation called simulation-by-exclusion.  It is based on the
idea of computing reduction of range of $N$ caused by excluding some
inputs from consideration rather than the entire range. The advantage
of this approach is that computing range reduction can be dramatically
simpler.

Here is simulation-by-exclusion in more detail. Suppose that one needs
to check if an erroneous output \pnt{z} is produced by $N$.  Suppose
that a set of inputs $K$ is excluded from consideration. Let $R$ be
the set of outputs that disappear from the range of $N$ due to
exclusion of inputs from $K$.

One can have two cases. The first case is that $\pnt{z} \not\in R$.
This means that either \pnt{z} is not in the range of $N$ i.e. $N$ is
correct or $N$ is buggy but there is an input \pnt{x} producing
\pnt{z} that is not in $K$. So exclusion of the inputs of $K$ does not
make \pnt{z} disappear from the range of $N$. Then regardless of
whether $N$ is buggy or not, one can safely remove the inputs of $K$
from further consideration. The second case is that $\pnt{z} \in R$.
Then \pnt{z} is in the range of $N$ and $K$ contains \ti{all} inputs
producing \pnt{z} i.e. all counterexamples. That is $N$ is
buggy. Simulation-by-exclusion can be used in many different
scenarios. In this paper, we consider some of them.



==> storage.tex <==
\subsection{CRR in terms of  noise sensitivity}
\label{subsec:crr_noise}
As we mentioned above, the CRR problem reduces to the problem of
Partial Quantifier Elimination (PQE).  In~\cite{hvc-14}, we showed how
one can solve the PQE problem using the machinery of dependency
sequents~\cite{fmcad12,fmcad13}. Importantly, a solution of the CRR
problem provided by a PQE solver is \ti{approximate}.  Let $Q$ be the
set of outputs disappearing from the range of circuit $N$ after a set
of inputs $K$ is excluded. A solution $Q^*$ returned by a PQE-solver
is a superset of $Q$ where $Q^* \setminus Q$ is ``noise'' consisting
of the outputs that are not in the range of $N$.

Since PQE solvers produce only approximate solutions to the CRR
problem, an important characteristic of a method based on CRR is its
sensitivity to noise. EC by CRR sketched above is an example of a
method that is \ti{noise-insensitive} while simulation-by exclusion is
\ti{noise-sensitive}. The reason why EC by CRR is noise-insensitive is
that the input constraints do not exclude any behaviors to be
verified. In this method of EC, one builds a circuit $M$ of
Figure~\ref{fig:two_indep} and eliminates the spurious behaviors where
$\pnt{x'}\neq \pnt{x''}$. The presence of a bug corresponds to the
situation when an erroneous output is \ti{not excluded} from the
range of $M$ under the input constraints. Adding noise can only
decrease the number of outputs of $M$ that are not excluded under
input constraints.


Conversely, simulation-by-exclusion is based on elimination of valid
inputs.  Then, the presence of a bug corresponds to the situation
where an erroneous output \pnt{z} is \ti{excluded} from the range of
$M$. In this case, the presence of noise is harmful: one does not know
if \pnt{z} is indeed excluded from the range of $M$ or it is noise
i.e. \pnt{z} is not in the range of $M$ at all. In
Subsection~\ref{subsec:sim_by_excl_and_crr}, we describe how to deal
with this problem.

